CROWN: Conversational Passage Ranking by Reasoning over Word Networks

Information needs around a topic cannot be satisfied in a single turn; users typically ask follow-up questions referring to the same theme and a system must be capable of understanding the conversational context of a request to retrieve correct answers. In this paper, we present our submission to the TREC Conversational Assistance Track 2019, in which such a conversational setting is explored. We propose a simple unsupervised method for conversational passage ranking by formulating the passage score for a query as a combination of similarity and coherence. To be specific, passages are preferred that contain words semantically similar to the words used in the question, and where such words appear close by. We built a word-proximity network (WPN) from a large corpus, where words are nodes and there is an edge between two nodes if they co-occur in the same passages in a statistically significant way, within a context window. Our approach, named CROWN, improved nDCG scores over a provided Indri baseline on the CAsT training data. On the evaluation data for CAsT, our best run submission achieved above-average performance with respect to AP@5 and nDCG@1000.

==> sections/backup.tex <==

\subsection{Scoring Candidate Passages}
In CROWN,
the final score of a passage consists of a weighted sum of three individual scores, namely the $nodescore$ (the similarity score calculated from the node weights), the $edgescore$ (the coherence score calculated from the edge weights) and the $indriscore$.
%, which is $\frac{1}{rank}$, where $rank$ is the rank the passage received by Indri. 
More formerly, the score for a passage $P_{i}$ is calculated as follows:
\[score = h_{1} \cdot indriscore + h_{2} \cdot nodescore + h_{3} \cdot edgescore\]  where $h_{1}$,  $h_{2}$ and  $h_{3}$ are hyperparameters.
The $nodescore$ is calculated in the following way:
\[nodescore = \sum_{j=1}^n \frac{\mathbb{1}_{C1(p_{i,j})} \times (\max_{k \in cq} sim(e(p_{i,j}), e(cq_{k})))}{NC}\] 
where $\mathbb{1}_{C1(p_{i,j}})$ maps to 1 if the condition $C1(p_{i,j})$ is fulfilled otherwise to 0 and $NC$ is the number of times the indicator function has the value $1$; $e(p_{i,j})$ is the word embedding of the j-th token in the i-th passage; $e(cq_{k})$ is the word embedding of the k-th token in the conversational query $cq$ and $sim$ denotes the cosine similarity between the passage token and the query token embeddings.   $C1(p_{i,j})$  is defined as
\[C1(p_{i,j}) = \exists cq_{k} \in cq: sim(e(p_{i,j}), e(cq_{k})) > NT\]
where $NT$ is a threshold for node similarity.
The $edgescore$ is calculated as follows:
\[edgescore= \sum_{j=1}^n \sum_{k=j+1}^{PROX}  \frac{\mathbb{1}_{C2(p_{i,j}, p_{i, k}}) \times NPMI(p_{i,j}, p_{i, k})}{EC}\]
where $PROX$ is the proximity window in which the two tokens should co-occur; $NPMI(p_{i,j}, p_{i, k})$ is the normalized point-wise
mutual information between j-th and the k-th token in the current passage, calculated from the MARCO corpus; $\mathbb{1}_{C2(p_{i,j}, p_{i, k}})$  maps to 1 if condition $C2(p_{i,j}, p_{i, k})$ is fulfilled otherwise to 0 and $EC$ is the number of times the indicator function has the value $1$; $C2(p_{i,j}, p_{i, k})$ is defined as:
\begin{align*}
%\begin{split}
C2(p_{i,j}, p_{i, k}) &= hasEdge(p_{i, j}, p_{i,k}) \\
    &\land NPMI(p_{i,j}, p_{i, k}) > ET \\
    &\land  (\exists cq_{r}, cq_{s} \in cq: (sim(e(p_{i,j}), e(cq_{r})) > NT 
    \land sim(e(p_{i,k}), e(cq_{s})) > NT)  \\
    &\land \not \exists  cq_{r'}, cq_{s'} \in cq:  
       sim(e(p_{i,j}), e(cq_{r'})) >  sim(e(p_{i,j}), e(cq_{r})) \\
            &\lor sim(e(p_{i,k}), e(cq_{s'})) >  sim(e(p_{i,k}), e(cq_{s})) ) \\
    &\land cq_{r} \neq cq_{s}
%\end{split}
\end{align*}
where $hasEdge$ returns true if there is an edge between the two tokens in the graph;  $ET$ is the edge threshold (only npmi values above this threshold are considered),
$cq$, $sim$ and $NT$ are defined in the same way as for the nodescore.  \\
Finally, the $indriscore$ is defined as follows:
\[indriscore = \frac{1}{rank} \] where $rank$ is the rank the passage received by Indri.  
